Adaptive Charging Networks: A Framework for Smart Electric Vehicle Charging

We describe the architecture and algorithms of the Adaptive Charging Network (ACN), which was first deployed on the Caltech campus in early 2016 and is currently operating at over 100 other sites in the United States. The architecture enables real-time monitoring and control and supports electric vehicle (EV) charging at scale. The ACN adopts a flexible Adaptive Scheduling Algorithm based on convex optimization and model predictive control and allows for significant over-subscription of electrical infrastructure. We describe some of the practical challenges in real-world charging systems, including unbalanced three-phase infrastructure, non-ideal battery charging behavior, and quantized control signals. We demonstrate how the Adaptive Scheduling Algorithm handles these challenges, and compare its performance against baseline algorithms from the deadline scheduling literature using real workloads recorded from the Caltech ACN and accurate system models. We find that in these realistic settings, our scheduling algorithm can improve operator profit by 3.4 times over uncontrolled charging and consistently outperforms baseline algorithms when delivering energy in highly congested systems.

==> sections/case_studies.tex <==
% !TEX root = ../main.tex

\section{Case Studies} \label{sec-case-studies}
To demonstrate the efficacy and flexibility of our online scheduling framework, we now consider a series of case studies. These case studies consider a variety of operator objectives which have been expressed by real site owners. All case studies are run using real data collected from the Caltech ACN. In addition, when considering profit maximization, we use realistic revenues and Southern California Edison's time-of-use rate schedule, making our case studies not only informative of our scheduling framework's performance, but also of the business potential of operating large-scale EV charging systems.

\subsection{Preliminaries}
\subsubsection{Data}
For these case studies we consider real data collected from the Caltech ACN as part of ACN-Data between May 1, 2018 and October 1, 2018. During this period our system served 10,415 charging sessions and delivered a total of 92.78 MWh of energy. Table \ref{tab:summary_stats} shows relevant summary statistics for this dataset. We also show the distribution of arrivals and departures in the system in Fig.~\ref{fig:arrival_departure_dist}. These distributions can help us understand when the system is likely to be highly loaded. In addition, the distribution of arrivals relative to the TOU rate schedule helps us to understand how much shifting is necessary to reduce energy costs in our system. All simulations were conducted using ACN-Sim \cite{lee_acnsim_2019}.

\begin{table}[t!]
\centering
\captionsetup{justification=raggedright}
\caption{\hspace{15pt} Average Statistics for EV Charging Test Cases Per Day\newline
May 1, 2018 - Oct. 1, 2018}\label{tab:summary_stats}

\renewcommand{\arraystretch}{1.1}
\begin{tabular}{l|c|c|c|c|c|}
\cline{2-6}
  & \begin{tabular}[c]{@{}c@{}}Mean\\Daily\\Sessions \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Mean\\Session\\Duration\\(hours)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Mean\\Session\\Energy\\(kWh)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Mean\\Daily\\Energy\\(kWh)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Max\\Concurrent\\Sessions\end{tabular}\\ \hline
\multicolumn{1}{|l|}{Sun} & 41.32 & 3.94 & 415.06 & 10.05 & 18\\
\multicolumn{1}{|l|}{Mon} & 71.00 & 6.14 & 677.13 & 9.54 & 42\\
\multicolumn{1}{|l|}{Tues} & 76.73 & 6.24 & 685.79 & 8.94 & 47\\
\multicolumn{1}{|l|}{Wed} & 75.45 & 6.22 & 660.16 & 8.75 & 44\\
\multicolumn{1}{|l|}{Thurs} & 78.50 & 5.96 & 665.21 & 8.47 & 42\\
\multicolumn{1}{|l|}{Fri} & 77.18 & 6.71 & 697.41 & 9.04 & 43\\
\multicolumn{1}{|l|}{Sat} & 43.32 & 5.01 & 439.59 & 10.15 & 18\\
\hline
\end{tabular}
\end{table}

\begin{figure}[t!]
\includegraphics[width = 0.8\columnwidth]{figs/Weekday_Arrival_Departure_Distribution_Oct_1.pdf}
\centering
\caption{Average arrivals and departures per hour for the period May 1, 2018 - Oct. 1, 2018. Background shading depicts the TOU rate at each time, with light grey, grey, and dark grey depicting off-peak, mid-peak, and peak pricing respectively. On weekdays we can see that most drivers arrive at the beginning of the morning mid-peak period and leave prior to the end of the peak period. Weekends, however have a much more uniform distribution of arrivals and departure owing to the heterogeneity of drivers weekend schedules.}
\label{fig:arrival_departure_dist}
\end{figure}

\subsubsection{Baseline Algorithms}
For comparison we consider a number of baseline algorithms which are included in ACN-Sim. These include Uncontrolled Charging, Round Robin (RR), Earliest Deadline First (EDF), Least-Laxity First (LLF), and Greedy Cost Minimization. In addition, we compare with the offline optimal to provide an upper bound on what any online algorithm could achieve. It is found by solving (\ref{eq:SCH.1}) with the relevant utility function and perfect knowledge of future arrivals. 

\subsubsection{Adaptive Scheduling Algorithm Setup}
For all case studies we consider the three-phase infrastructure present in the Caltech ACN. We set the length of each time slot, $\delta$, to 5 minutes and consider a maximum optimization horizon of 12 hours. For all cases except those in Section~\ref{sec:practical_considerations} we do not consider a maximum recompute period, $P$, as we use an ideal battery management system model for these tests and EVs are assumed to follow the control signal exactly. In Section~\ref{sec:practical_considerations} we use more realistic models and set $P=5$ minutes.

\subsection{Energy Delivery in Oversubscribed Infrastructure}
In our first case study we consider the objective of maximizing total energy delivered. This objective is used when the operator's primary goal is driver satisfaction or when profit per unit energy at a site is constant. In these cases the primary purpose of adaptive scheduling is to meet driver demand with minimal infrastructure investment. To satisfy this operator objective we use the Adaptive Scheduling Algorithm (Alg. \ref{alg:MPC}) with utility function

\begin{equation}
    U^\mathrm{QC} := V^{QC} + 10^{-14}V^{ES}
\end{equation}

Here $U^{QC}$ encourages the system to deliver as much energy as possible as quickly as possible which helps to free capacity for future arrivals.
We refer to this algorithm as SCH-Quick Charge (SCH-QC).

In order to demonstrate the effect of highly constrained infrastructure, we vary the capacity of transformer $t_1$ between 0 and 100 kW. For reference, the actual transformer in our system is 150 kW and a conventional system for \numevse{} 7kW EVSEs would require 378 kW of capacity. We then measure what percent of the total energy demand can be met using SCH-QC as well as four baseline scheduling algorithms and the offline optimal. The results of this test are shown in Fig.~\ref{fig:energy_delivered_const_infra}.

From Fig.~\ref{fig:energy_delivered_const_infra} we can see that SCH-QC performs near optimally in terms of the percent of demand met and with it we are able to meet 100\% of driver demand with just 70 kW of transformer capacity even in the online setting. Meanwhile other baseline algorithms struggle in highly constrained infrastructure.

\zach{This section is interesting but less relevant, so we could remove it.}Among the baselines algorithms, we note that RoundRobin outperforms the other baselines for extremely low transformer capacities. This is because RoundRobin is able better balance between phases which the sorting based methods do not consider. As capacity increases, however, EDF and LLF outperform RoundRobin, as prioritizing drivers by their energy demands and deadline becomes more important than squeezing out capacity from the system. SCH-QC is able to factor in driver demands and deadlines while also balancing phases, which helps to explain its superior performance.

\begin{figure}[t!]
\includegraphics[width=\columnwidth]{figs/GreedyInfrastructureDerate}
\centering
\caption{Percentage of driver's energy demands which can be met at varying capacities for transformer $t_1$ for the month of Sept. 2018. Here demand met is defined as the ratio of total energy delivered to total energy requested.
}
\label{fig:energy_delivered_const_infra}
\end{figure}

\subsection{Profit Maximization with TOU Rates}\label{sec:case-no-dc}
We next consider the case where an operator would like to maximize their profit subject to time-of-use electricity tariffs. For this case study we adopt the Southern California Edison TOU rate schedule for separately metered EV charging systems between 20-500~kW which is shown in Table~\ref{tab:tou_rates} \cite{choi_general_2017}. We do not, however, consider a demand charge for this case, as we will do so in the next case study. We consider a fixed revenue of \$0.30 / kWh.\footnote{While this may seem high, it is actually reasonable as it can be sourced not only from the driver but also from subsidies and by selling credits in carbon markets such as the California Low-Carbon Fuel Standard program which is currently trading at the equivalent of \$0.14~/~kWh as of Oct. 2018.}

\renewcommand{\arraystretch}{1.1}
\begin{table}[t!]
\centering
\captionsetup{justification=raggedright}
\caption{\hspace{15pt} SCE TOU Rate Schedule for EV Charging}\label{tab:tou_rates}
\begin{tabular}{c|c|}
\cline{2-2}
\multicolumn{1}{l|}{}                               & Rates                \\ \hline
\multicolumn{1}{|c|}{On-Peak (12pm-6pm)}            & \$0.25 / kWh         \\ \hline
\multicolumn{1}{|c|}{Mid-Peak (8am-12pm, 6pm-11pm)} & \$0.09 / kWh         \\ \hline
\multicolumn{1}{|c|}{Off-Peak (11pm-8am)}           & \$0.06 / kWh         \\ \hline
\multicolumn{1}{|c|}{Demand Charge}                 & \$15.48 / kW / month \\ \hline
\end{tabular}
\end{table}

To facilitate maximizing profits considering only energy charges, we propose two algorithms based on \textbf{SCH}. The first, denoted SCH-Energy Charge (SCH-EC), uses the utility function
\begin{equation}
    U^\mathrm{EC} := V^{EC} + 10^{-14}V^{ES}
\end{equation}

\noindent and the second, denoted SCH-Energy Charge Quick (SCH-ECQ) uses

\begin{equation}
    U^\mathrm{ECQ} := V^{EC} + 10^{-4}V^{QC} + 10^{-14}V^{ES}
\end{equation}

We add the $V^{QC}$ term to SCH-ECQ in order to free capacity for future arrivals by encouraging charging early in each rate period. Since rates are flat during each period, we can front load charging within a period without increasing energy costs.

We consider the profit gained by our algorithms as well as the baselines for the five month period beginning in May 2018. The results of this test are shown in Fig.~\ref{fig:profit_max_no_dc}. Here we can see that Uncontrolled, FCFS, and Round Robin perform poorly relative to the optimal.\footnote{Somewhat surprisingly uncontrolled charging generates higher profits than FCFS and Round Robin. This is because uncontrolled charging does not have to contend with infrastructure limits. This, combined with the arrival patterns shown in Fig.~\ref{fig:arrival_departure_dist}, means that uncontrolled charging is able to deliver more energy during mid-peak (rather than on-peak) hours than FCFS or Round Robin.} This is expected, as these algorithms do not consider pricing signals at all. The IndividualGreedy algorithm does quite well in this test, achieving 98.7\% of the optimal profit available. However, the algorithms we propose based on our framework perform even better, achieving 99.58\% and 99.99\% for SCH-EC and SCH-ECQ respectively. As expected SCH-ECQ out-performs SCH-EC.

\begin{figure}[t!]
\includegraphics[width = \columnwidth]{figs/ProfitMaxNoDC.pdf}
\centering
\caption{Operator profit achieved via various scheduling approaches when using SCE's TOU rate schedule without demand charge.
}
\label{fig:profit_max_no_dc}
\end{figure}

\subsection{Profit Maximization with Demand Charge}\label{sec:pm_w_dc}
We next consider the more difficult task of maximizing profit in the presence of TOU rates and demand charge. We still consider the same rate schedule in Table~\ref{tab:tou_rates}, but now with the additional demand charge component. Demand charges are assessed on the maximum power draw of a customer over the billing period which we assume to be one month. These charges can be very high, especially in uncontrolled EV charging systems where many drivers might arrive in close succession and charge at concurrently leading to high peak demand.

\begin{figure}[t!]
\includegraphics[width = \columnwidth]{figs/ProfitMaxDcCombined}
\centering
\caption{Operator profit achieved via various scheduling approaches when using SCE's TOU rate schedule with demand charge.}
\label{fig:profit_max_dc}
\end{figure}

To demonstrate the importance of considering demand charge when scheduling, we can evaluate the profit of scheduled found by SCH-EC and SCH-ECQ when including demand charge. This is shown in Fig.~\ref{fig:profit_max_dc}. Here we can see that demand charge was reduced the profit obtained by SCH-EC and SCH-ECQ by 55\% and 60\% respectively. Moreover, these algorithms under perform the optimal by 35\% and 45\% respectively. Note that when demand charge is considered, SCH-ECQ performs worse than SCH-EC. This is because SCH-ECQ leads to higher peaks in demand. We also note that the baseline algorithms we consider also perform poorly when demand charge is considered. This is especially true of uncontrolled charging, which leads to high peaks in demand which severely reduces profitability.

This motivates us to consider demand charge in our scheduling problem. To do this we use the utility function\footnote{Note that while SCH-ECQ fared worse than SCH-EC when considering demand charge, we still include $V^{QC}$ in this formulation. This is because $V^{DC}$ will enforce a low peak, so we can still use $V^{QC}$ to encourage charging quickly when possible.}
\begin{equation}
    U^\mathrm{DC} := V^{DC} + 10^{-4}V^{QC} + 10^{-14}V^{ES}
\end{equation}

Here $V^{DC}$ as two tunable parameters the demand charge proxy,  $\hat{\Delta}$, and the previous/projected peak demand, $L_0^{max}$. Careful selection of these parameters is necessary as demand charge is a ratcheting cost which must be considered over the entirety of the billing period. Meanwhile, the ASA framework is designed to work on small sub-intervals of this period. If we try to naively include demand charge into our objective by setting $\hat{\Delta}$ to the equivalent of \$15.48 / kW and $L_0^{max}=0$, no charging would occur as the marginal cost of increasing peak demand would be far greater than the marginal benefit of charging the EVs.

To account for this we consider three parameter configurations. The first we call SCH-Demand Charge Proportional (SCH-DCP). In this configuration we scale the true demand charge, $\Delta$, by the percentage of the billing period which is covered by the optimization horizon to arrive at $\hat{\Delta}$. In this case we begin the billing period with $L^{max}_0=0$ then update it, prior to each iteration, to be the highest peak so far in the billing cycle. We see in Fig.~\ref{fig:profit_max_dc} that this results in a significant improvement over not considering demand charge at all, but still achieves only 84.5\% of the optimal profit available. By examining the schedules produced by SCH-DCP, we see that while it achieves lower energy costs that the optimal, it has a much higher demand charge. This is likely because $\hat{\Delta}$ is too low.

To address this, we can instead prorate the demand charge on a daily basis, e.g. $\hat{\Delta} := \Delta / 30$. We denote this configuration SCH-Demand Charge Daily (SCH-DCD). The intuition behind this change is that usage in our system is extremely low overnight. Thus the scheduling algorithm should at least consider the demand charge it will generate over a full 24 hour period. We see in Fig.~\ref{fig:profit_max_dc} that this change increases performance to be within 93.6\% of optimal.

While SCH-DCD offers good performance, there is still room for improvement. We note that selecting the correct peak usage is extremely important to maximizing profit. So rather than using a demand charge proxy, we consider what would happen if we knew a-priori what the optimal peak from the offline case would be.
%We can find this optimal peak after the fact by solving OfflineOptimal for the current month and extracting the peak usage.
We could then set $L_0^{max}$ to be this optimal peak current and $\hat{\Delta}=\Delta$. We denote this configuration SCH-Demand Charge Oracle (SCH-DCO) since we rely on an oracle to supply the optimal peak. We can see in Fig.~\ref{fig:profit_max_dc} that SCH-DCO performs near optimally (within 99.6\%).

However, in practice, we do not have access to an oracle to provide the optimal peak demand, so we cannot use SCH-DCO directly. We must instead predict the optimal peak. One way to do so is to run OfflineOptimal over the previous 28 day period and use the resulting peak as an estimate of the optimal peak. We repeat this procedure daily (at midnight), so that the algorithm is able to adapt to changing usage patterns. At the beginning of each day, we set $L_0^{max}$ to be the max of the peak usage so far in that billing period and our estimate of the optimal peak. We denote this configuration SCH-Demand Charge Reflective (SCH-DCR). In Fig.~\ref{fig:profit_max_dc} we can see that SCH-DCR is very close to optimal, achieving  97.7\% of the available profit.

While SCH-DCR is able to outperform SCH-DCD, there is still a trade-off between the two. First, SCH-DCD does not require access to historical system usage. This is important for new sites and for sites which do not wish to store past usage. Second, the two algorithms have very different behavior during high usage periods. Because SCH-DCR essentially fixes its peak using historical data, some vehicles will not be charged if doing so would violate this peak. Meanwhile, SCH-DCD has a much lower bar for raising its peak usage, meaning that more of the EV demand would be met but at higher cost over the entire billing period. Thus when choosing between the two, the site operator should consider which behavior better aligns with their goals.\footnote{It is also possible to run both algorithms with an equality energy constraint, which would mean that the demand for all drivers would be met. However, doing this in practice could lead to incredibly high costs for the operator.}

\subsection{Practical Considerations} \label{sec:practical_considerations}
In previous case studies we have ignored some of the more difficult issues which arise from practical EV charging systems, namely non-ideal battery behavior and additional (discrete) constraints on individual charging rates. In this section we address the effect of incorporating these constraints into our scheduling problem.

We once again consider the problem of profit maximization with demand charge. We use the best practical algorithm we have considered, SCH-DCR, as a base and measure performance relative to the profit achieved in the previous section where ideal EV and EVSE models were used. The effect of including these practical EV and EVSE considerations on the operator's profit are shown in Fig.~\ref{fig:practical_considerations}.

\begin{figure}[t!]
\includegraphics[width = \columnwidth]{figs/PracticalConsiderations}
\centering
\caption{Operator profit achieved when considering practical EV charging models as a percent of profit when considering ideal EV and EVSE models. Profits are aggregated over June 1 through Oct. 1.
}
\label{fig:practical_considerations}
\end{figure}

\subsubsection{Non-ideal battery behavior}
We first address the effects of non-ideal battery behavior. We consider a two-stage battery charging model. The first stage, referred to as \emph{bulk} charging, occurs up to 80\% state of charge. In this stage current draw, neglecting changes in pilot, is near constant. The second stage, called \emph{absorption}, finishes charging the remaining 20\%. In this stage, current decreases as the battery reaches full charge. To simulate this we use the Linear2Stage battery model included in ACN-Sim \cite{lee_acnsim_2019}.

We account for this non-ideal battery behavior by computing a new solution to our scheduling problem periodically. This allows our algorithm to update its schedule to account for deviations from the assigned charging rates caused by battery behavior. For this test we set the minimum recompute period to be equal to the length of one period, 5 minutes. From Fig.~\ref{fig:practical_considerations} we see that non-ideal battery behavior leads to approximately a 5.3\% reduction in operator profit.

\subsubsection{Charging rate restrictions}
We next consider the limitations on charging rate imposed by EVSEs and battery management systems. As mentioned in Section \ref{sec:key-insights} most EVSEs on the market, including those used in our ACN testbed, provide only a discrete set of allowable pilot signals. For this test we use $\rho := \{0, 6, 7, ..., 31, 32\}$, which is the allowable rate set for AeroViroment EVSEs. In addition, the J1772 standard forbids charging rates in the range of 0-6 A and experience has shown us that some EVs do not recover after being assigned at 0 A pilot signal, meaning EVs should receive at least a 6 A pilot from when they plug in until their demand is met. These factors motivate the post-processing heuristic described in Section \ref{sec:post_processing}.

To demonstrate the effect of accounting for these restrictions on operator profit, we first run SCH-DCR then run the resulting schedule through our post-processing steps (\ref{eq:post_processing}) and (\ref{eq:rate_projection}) with $\gamma = 10^{-2}$. We once again set the maximum recompute period to be 5 minutes (1 period) so that SCH-DCR is able to account for deviations caused by the post-processing. From Fig.~\ref{fig:practical_considerations} we see that accounting for charging rate restrictions using the post-processing approach we propose leads to approximately a 10\% reduction in operator profit.

\subsubsection{Practical model}
In practice we must contend with both non-ideal battery behavior and rate restrictions. As such, in our final scenario we consider both factors simultaneously. The result, as seen in Fig.\ref{fig:practical_considerations}, is an approximately 12.5\% reduction in operator profit relative to SCH-DCR with the ideal EV/EVSE model. This demonstrates that our proposed algorithms are robust when applied to more realistic models of EV and EVSE behavior and capabilities.
\zach{It would be nice to formulate the offline optimal problem as a mixed integer program and solve. But I don't know if this is feasible.}

==> sections/network_model.tex <==
Infrastructure limits are indexed by $j\in \hat{\mathcal{R}}$. 
For each constraint $j$ and time $t$, the magnitude of current $R_j(t) \in \mathbb{C}$ must be less than the limit $\bar{R}_j(t)$. Let $A \in \mathbb{R}^{MxN}$ define the linear relationship between the current phasor of each EVSE, $I_k(t) := i_k(t)e^{j\phi_k}$, and the aggregate currents $R(t) = [R_1(t), ..., R_M(t)]$, i.e. $A^{T}I(t) = R(t)$. We can then express the infrastructure constraints as
\begin{equation}\label{eq:inf_constraints}
    |R_j(t)| = \left|\sum_{k\in\mathcal{V}} a_{jk} I_k(t) \right| \leq \bar{R}_j(t) \quad t \in \mathcal{T}, j \in \hat{\mathcal{R}}
\end{equation}

These can be expressed as second-order cone constraints and are thus convex and can be handled by many off-the-shelf solvers. Some applications, however, even these SOC constraints are too computationally expensive. Simpler, but more conservative constraints can be derived by observing
\begin{equation*}
    |R_j(t)| = \left|\sum_{k\in\mathcal{V}} a_{jk} I_k(t) \right| \leq \sum_{k\in\mathcal{V}} |a_{jk}| i_k(t) 
\end{equation*}
% 
This yields affine constraints in the form
\begin{equation}\label{eq:inf_constraints_affine}
    |R_j(t)| \leq \sum_{k\in\mathcal{V}} |a_{jk}| i_k(t) \leq \bar{R}_j(t) \quad t \in \mathcal{T}, j \in \hat{\mathcal{R}}
\end{equation}
% 
Note that if all EVSEs are on a single phase, e.g. $\phi_1 = \phi_k \ \forall k$, then (\ref{eq:inf_constraints_affine}) is equivalent to (\ref{eq:inf_constraints}).

